Mining gold from implicit models to improve likelihood-free inference

Simulators often provide the best description of real-world phenomena. However, they also lead to challenging inverse problems because the density they implicitly define is often intractable. We present a new suite of simulation-based inference techniques that go beyond the traditional Approximate Bayesian Computation approach, which struggles in a high-dimensional setting, and extend methods that use surrogate models based on neural networks. We show that additional information, such as the joint likelihood ratio and the joint score, can often be extracted from simulators and used to augment the training data for these surrogate models. Finally, we demonstrate that these new techniques are more sample efficient and provide higher-fidelity inference than traditional methods.

==> babelbst.tex <==
%%
%% This is file `merlin.tex',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% merlin.mbs  (with options: `bblbst')
%% 
%% IMPORTANT NOTICE:
%% 
%% For the copyright see the source file.
%% 
%% Any modified versions of this file must be renamed
%% with new filenames distinct from merlin.tex.
%% 
%% For distribution of the original source see the terms
%% for copying and modification in the file merlin.mbs.
%% 
%% This generated file may be distributed as long as the
%% original source files, as listed above, are part of the
%% same distribution. (The sources need not necessarily be
%% in the same archive or directory.)
%% Copyright 1994-2011 Patrick W Daly
 % ===============================================================
 % IMPORTANT NOTICE:
 % This bibliographic style (bst) file has been generated from one or
 % more master bibliographic style (mbs) files, listed above.
 %
 % This generated file can be redistributed and/or modified under the terms
 % of the LaTeX Project Public License Distributed from CTAN
 % archives in directory macros/latex/base/lppl.txt; either
 % version 1 of the License, or any later version.
 % ===============================================================
 % Name and version information of the main mbs file:
 % \ProvidesFile{merlin.mbs}[2011/11/18 4.33 (PWD, AO, DPC)]
 % This is babelbst.tex for English.
 % It should serve as a model for other languages.
 % Alternatively, store it under a different name (e.g. englbst.tex)
 % and then \input it with a command in babelbst.tex.
\def\bbland{and}                \def\bbletal{et~al.}
\def\bbleditors{editors}        \def\bbleds{eds.}
\def\bbleditor{editor}          \def\bbled{ed.}
\def\bbledby{edited by}
\def\bbledition{edition}        \def\bbledn{edn.}
\def\bblvolume{volume}          \def\bblvol{vol.}
\def\bblof{of}
\def\bblnumber{number}          \def\bblno{no.}
\def\bblin{in}
\def\bblpages{pages}            \def\bblpp{pp.}
\def\bblpage{page}              \def\bblp{p.}
\def\bbleidpp{pages}
\def\bblchapter{chapter}        \def\bblchap{chap.}
\def\bbltechreport{Technical Report}
\def\bbltechrep{Tech. Rep.}
\def\bblmthesis{Master's thesis}
\def\bblphdthesis{Ph.D. thesis}
\def\bblfirst{First}            \def\bblfirsto{1st}
\def\bblsecond{Second}          \def\bblsecondo{2nd}
\def\bblthird{Third}            \def\bblthirdo{3rd}
\def\bblfourth{Fourth}          \def\bblfourtho{4th}
\def\bblfifth{Fifth}            \def\bblfiftho{5th}
\def\bblst{st}  \def\bblnd{nd}  \def\bblrd{rd}
\def\bblth{th}
\def\bbljan{January}  \def\bblfeb{February}  \def\bblmar{March}
\def\bblapr{April}    \def\bblmay{May}       \def\bbljun{June}
\def\bbljul{July}     \def\bblaug{August}    \def\bblsep{September}
\def\bbloct{October}  \def\bblnov{November}  \def\bbldec{December}
\endinput
%%
%% End of file `merlin.tex'.


==> figures/graphical-model.tex <==
%\begin{figure}
%	\centering
%%	\begin{subfigure}{0.4\textwidth}
%		\centering
\scalebox{1.0}{
\begin{tikzpicture}

% Define nodes
\node[latent]                             (zlt) {$z_{t}$};
%\node[const, xshift=1.75cm, above=1.75cm of zlt]             (theta) {$\theta\;$};
\node[obs, right=2.5cm of zlt]             (x) {$x$};


%\factor[above= of zlt, yshift=0.4cm] {policy} {above,xshift=0.07cm:$\pi_\theta(z_t | z_{<t})$} {} {};
%\factor[above= of zlt, yshift=0.4cm] {policy} {above,xshift=0.07cm:$p(z_t | z_{<t}, \theta)$} {} {};
\factor[above= of zlt, yshift=0.4cm] {policy} {above,xshift=0.07cm:$\pi_\theta(z_t | z_{<t})$} {} {};

%\factor[right= of zlt, xshift=1.cm] {observe} {above,xshift=0.07cm:$p_\theta(x | z)$} {} {};
%\factor[right= of zlt, xshift=1.cm] {observe} {below,xshift=-0.1cm:$p_\theta(x | z)$} {} {};
%\factor[right= of zlt, xshift=1.cm] {observe} {below,yshift=0.05cm,xshift=-0.1cm:$p(x | z, \theta)$} {} {};
\factor[right= of zlt, xshift=1.cm] {observe} {below,yshift=0.05cm,xshift=-0.1cm:$p_\theta(x | z)$} {} {};

\node[const, above=1.cm of observe]             (theta) {$\theta$};
%\node[const, right=2.cm of theta]             (theta1) {$\theta_1$};


%\factor[above= of zlt, yshift=0.1cm] {policy} {left,xshift=0.07cm:$\pi_\theta(z_t | z_{<t})$} {zlt} {zlt};
%\factor[below= of L, yshift=-0.1cm] {sum} {left,xshift=0.07cm:$+$} {zt} {zlt};

\edge[shorten <=0.1cm] {theta} {policy} ;
\edge[shorten <=0.1cm] {theta} {observe} ;
\edge {zlt} {x} ;
%\draw [->,>={triangle 45}] (zlt) .. controls (0.5,1.3) and (-0.5,0).. (zlt);
\draw [-,>={triangle 45}] (zlt) .. controls (1,0) and (1.,1.3).. (policy);
%\draw [->,>={triangle 45}] (policy) .. controls (-1,1) and (-1.,0.5).. (zlt);
\draw [->,>={triangle 45}] (policy) .. controls (-1,1.3) and (-1.,0).. (zlt);


\node[det, below=of zlt]                             (txz) {$\;t(x,z | \theta)\;$};
\node[det, below=of x]                             (rxz) {$\;r(x,z | \theta, \theta_1)\;$};

\node[const, right=.7cm of rxz]             (theta1) {$\theta_1$};

\edge[shorten <=0.1cm] {theta} {txz} ;
\edge[shorten <=0.1cm] {theta} {rxz} ;
\edge[shorten <=0.1cm] {theta1} {rxz} ;

%\edge {theta} {txz} ;
\edge {x} {txz} ;
\edge {zlt} {txz} ;
\edge {x} {rxz} ;
\edge {zlt} {rxz} ;


\end{tikzpicture}
}
%		\caption{A graphical model representation of a density defined implicitly by a stochastic scientific simulator where the latent state $z_t$ evolves sequentially according to a policy $p(z_t | z_{<t}, \theta)$ and final observation model $p(x|z, \theta)$. The joint score and marginal score are deterministic functions derived from the implicit density.}
%		\label{fig:samples}
%%	\end{subfigure}
%\end{figure}

